Verified Implementation of an Efficient Term-Rewriting Algorithm for Multiplier Verification on ACL2

Automatic and efficient verification of multiplier designs, especially through a provably correct method, is a difficult problem. We show how to utilize a theorem prover, ACL2, to implement an efficient rewriting algorithm for multiplier design verification. Through a basic understanding of the features and data structures of ACL2, we created a verified program that can automatically verify various multiplier designs much faster than the other state-of-the-art tools. Additionally, users of our system have the flexibility to change the specification for the target design to verify variations of multipliers. We discuss the challenges we tackled during the development of this program as well as key implementation details for efficiency and verifiability. Those who plan to implement an efficient program on a theorem prover or those who wish to implement our multiplier verification methodology on a different system may benefit from the discussions in this paper.

==> eptcsdata.tex <==
\providecommand{\firstpage}{116}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.11}{10.4204/EPTCS.359.11}}
\pdfoutput=1

